Firefly: Supporting Drone Localization With Visible Light Communication

Drones are not fully trusted yet. Their reliance on radios and cameras for navigation raises safety and privacy concerns. These systems can fail, causing accidents, or be misused for unauthorized recordings. Considering recent regulations allowing commercial drones to operate only at night, we propose a radically new approach where drones obtain navigation information from artificial lighting. In our system, standard light bulbs modulate their intensity to send beacons and drones decode this information with a simple photodiode. This optical information is combined with the inertial and altitude sensors in the drones to provide localization without the need for radios, GPS or cameras. Our framework is the first to provide 3D drone localization with light and we evaluate it with a testbed consisting of four light beacons and a mini-drone. We show that, our approach allows to locate the drone within a few decimeters of the actual position and compared to state-of-the-art positioning methods, reduces the localization error by 42%.

==> sections/SoA.tex <==
\section{State of the art} %Yanqiu
Comparison with SoA\\
Taxonomy: Tx complexity vs Rx complexity\\
Focus on the quadrant of interest and discard complex algorithms.\\
Show accuracy (nice plot)\\
Consider LED Density and other aspects of the comparison such as power of transmitter, quality of PDs, etc...
